Canonical Formulation of Spin in General Relativity

The present thesis aims at an extension of the canonical formalism of Arnowitt, Deser, and Misner from self-gravitating point-masses to objects with spin. This would allow interesting applications, e.g., within the post-Newtonian (PN) approximation. The extension succeeded via an action approach to linear order in the single spins of the objects without restriction to any further approximation. An order-by-order construction within the PN approximation is possible and performed to the formal 3.5PN order as a verification. In principle both approaches are applicable to higher orders in spin. The PN next-to-leading order spin(1)-spin(1) level was tackled, modeling the spin-induced quadrupole deformation by a single parameter. All spin-dependent Hamiltonians for rapidly rotating bodies up to and including 3PN are calculated.

==> erklaerung.tex <==
\mychapters{Ehrenwörtliche Erklärung}
\currentpdfbookmark{Ehrenwörtliche Erklärung}{erkl}
% \newpage
% \pagestyle{plain}
% {\usekomafont{disposition}\usekomafont{chapter}Ehrenwörtliche Erklärung}\vspace{0.7cm}\\

Ich erkläre hiermit ehrenwörtlich, dass
\begin{itemize}
 \item mir die geltende Promotionsordnung der Physikalisch-Astronomischen
	Fa\-kul\-tät vom 21.01.2009 bekannt ist;
 \item ich die Dissertation selbst angefertigt habe, unter Angabe aller
	benutzter Hilfsmittel, persönlicher Mitteilungen und Quellen,
	sowie unter Kennzeichnung aller Textabschnitte eigener Prüfungsarbeiten
	oder eines Dritten;
\item alle Personen, die mich bei der Auswahl und Auswertung des Materials sowie
	bei der Herstellung des Manuskripts unterstützt haben in der Danksagung
	(Acknowledgments) benannt wurden und keine weiteren Personen an der
	inhaltlich-materiellen Erstellung der vorliegenden Arbeit beteiligt waren;
\item Dritte weder unmittelbar noch mittelbar geldwerte Leistungen von
	mir für den Inhalt der vorgelegten Dissertation betreffende Arbeiten
	erhalten haben, sowie die Hilfe eines Promotionsberaters nicht in
	Anspruch genommen wurde;
\item die vorliegende Dissertation von mir weder im In- noch im Ausland als Prü\-fungs\-ar\-beit für eine
	staatliche oder andere wissenschaftliche Prüfung eingereicht wurde;
\item die gleiche, eine in wesentlichen Teilen ähnliche oder eine andere
	Dissertation von mir weder im In- noch im Ausland einer anderen
	Hochschule vorgelegt wurde.
\end{itemize}
Ich versichere ehrenwörtlich, dass ich nach bestem Wissen die reine Wahrheit gesagt und nichts verschwiegen habe.

\vspace{2cm}

\noindent
Jena, den \today\\
$\left. \right.$ \hfill $\overline{\qquad\qquad\text{Jan Steinhoff}\qquad\qquad}$

